Intelligent Software Tooling for Improving Software Development

Software has eaten the world with many of the necessities and quality of life services people use requiring software. Therefore, tools that improve the software development experience can have a significant impact on the world such as generating code and test cases, detecting bugs, question and answering, etc., The success of Deep Learning (DL) over the past decade has shown huge advancements in automation across many domains, including Software Development processes. One of the main reasons behind this success is the availability of large datasets such as open-source code available through GitHub or image datasets of mobile Graphical User Interfaces (GUIs) with RICO and ReDRAW to be trained on. Therefore, the central research question my dissertation explores is: In what ways can the software development process be improved through leveraging DL techniques on the vast amounts of unstructured software engineering artifacts?

==> abstract.tex <==
\begin{large}
\noindent 
\begin{flushleft}
Software has eaten the world with many of the necessities and quality of life services people use requiring software. Therefore, tools that improve the software development experience can have a significant impact on the world such as generating code and test cases, detecting bugs, question and answering, \etc~\new{ The success of Deep Learning (DL) over the past decade has shown huge advancements in automation across many domains, including Software Development processes. One of the main reasons behind this success is the availability of large datasets such as open-source code available through GitHub or image datasets of mobile Graphical User Interfaces (GUIs) with RICO \cite{Deka:UIST'17} and ReDRAW \cite{Moran2018} to be trained on. Therefore, the central research question my dissertation explores is: \textit{In what ways can the software development process be improved through leveraging DL techniques on the vast amounts of unstructured software engineering artifacts?}}


% can large amounts of unstructured data be leveraged to improve the software development process?}
% The integration of into developer workflows has created what we've coined as \textit{Intelligent Software Tools}.}

% Deep learning's success over the past decade has shown a potential method for helping with the creation of what we've coined \textit{Intelligent Software Tools}. Specifically, tools that automate or improve aspects of a software developer's workflow leveraging deep learning.
% One of the potential 
% Deep learning's success over the past decade has improved automation in many domains, including Software Engineering and has therefore positioned it to help improve software tooling.
\end{flushleft}

% 1. SLR
% 2. Tango
% 3. Athena
% 4. Completeformer

\begin{flushleft}

\new{We coin the approaches that leverage DL to automate or augment various software development task as \textit{Intelligent Software Tools}.} To guide our research of these intelligent software tools, we performed a systematic literature review to understand the current landscape of research on applying DL techniques to software tasks and any gaps that exist.
%This involved processing \nonsamplingtotal papers manually to extract information such as the software engineering task and deep learning model used.
\new{From this literature review, we found code generation to be one of the most studied tasks with other tasks and artifacts such as impact analysis or tasks involving images and videos to be understudied. Therefore, we set out to explore the application of DL to these understudied tasks and artifacts as well as the limitations of DL models under the well studied task code completion, a subfield in code generation.}
% artifacts such as images and videos to be understudied. With these results in mind, we set out to 
% were the most popular such as code generation or program synthesis.
% Therefore, for our efforts in developing intelligent software developer tooling, we wished to explore other potential software engineering tasks and artifacts.
Specifically, we developed a tool for automatically detecting duplicate mobile bug reports from user submitted videos. We used the popular Convolutional Neural Network (CNN) to learn important features from a large collection of mobile screenshots. Using this model, we could then compute similarity between a newly submitted bug report and existing ones to produce a ranked list of duplicate candidates that can be reviewed by a developer.
% This is done by first training a large deep learning model, we used the popular Convolutional Neural Network (CNN), to learn important features from a large collection of mobile screenshots. This model is then used to extract the important features from the frames in a user submitted video-based bug report. The features are then compared between a newly submitted video and a corpus of existing ones from previous bug reports to determine their similarity and produce a ranked list of duplicate candidates that a developer can review for duplicates.
Next, we explored impact analysis, a critical software maintenance task that identifies potential adverse effects of a given code change on the larger software system. \new{To this end, we created Athena, a novel approach to impact analysis that integrates knowledge of a software system through its call-graph along with high-level representations of the code inside the system to improve impact analysis performance.}
%Concretely, we explore extending state-of-the-art approaches in code representation that leverage the popular Transformer architecture \cite{vaswani2017attention} by injecting the call-graph information using a embedding propagation strategy inspired by Graph Convolutional Networks (GCNs) \cite{kipf2016semi}.}
% Therefore, we created \athena, a software tool that leverages knowledge of a software system through its call-graph when constructing a high-level representation of the methods inside of the system thereby allowing for information the role of the method to be taken into consideration when using the representation to perform code search via cosine similarity. We used a combination of the Transformer architecture \cite{Vaswani:NeurIPS2017}, which is a state of art model in natural language processing (NLP), and Node2Vec architecture \cite{node2vec-kdd2016}, which also is a popular model in Graph learning tasks.
Lastly, we explored the task of code completion, which has seen heavy interest from industry and academia \cite{hindle2016naturalness, tu2014localness, hellendoorn2019code, raychev2014code, bruch2009learning, jin2018hidden, izadi2022codefill, aye2021learning, Hellendoorn2017, hou2010towards, nguyen2019combining, robbes2008program, robbes2010improving, svyatkovskiy2021fast, svyatkovskiy2019pythia, yang2017language, chen2021evaluating, ciniselli2021empirical, github}. Specifically, \new{we explored various methods that modify the positional encoding scheme of the Transformer architecture for allowing these models to incorporate longer sequences of tokens when predicting completions than seen during their training as this can significantly improve training times.}
% Having a model that can be trained on shorter sequences and then later tested on longer sequences without a huge impact to performance has a number of advantages, namely in being able to decrease the cost of training since the standard self-attention mechanism the Transformer utilizes has a quadratic memory consumption based on the sequence length. Concretely, we explored whether the lessons learned from natural language processing could be extended to code.}

% Above, the abstract says "code generation" is well studied and this dissertation explores understudied tasks/artifacts, yet here we explored code completion which is well studied as well.  Focusing on code completion may require further justification or change the argument above: we focused on two understudied tasks (duplicate detection and impact analysis) and explored the limitations/benefits of DL models under well studied task (code completion) 

% two deep learning architectures, T5 \cite{raffel2020exploring} and ALiBi \cite{press2022alibi}, both of which have shown an interesting ability to be trained on short natural language English sequences yet perform well on sequences there are much longer during inference. We sought to answer whether these approaches could be applied to code as this could significantly decrease the cost of training these models.

% Next, we explored the applicability of recent state of the art language models for autocompleting code for developers. This involved evaluating different Transformer models, which have revolutionized the Natural Language Processing (NLP) domain, on autocompletion. Specifically, we investigated pure encoder and sequence to sequence Transformers and found that sequence to sequence Transformers perform extremely well compared to previous methods such as n-grams and Recurrent Neural Networks (RNNs). Additionally, we exploited recent advancements in multi-task training with the same sequence to sequence Transformer model to create a single deep learning model capable of performing many software engineering tasks, \ie autocompletion, program repair, assert case generation, \etc. 

% , exploited recent advancements in multi-task training to create a single deep learning model capable of performing many software engineering tasks from autocompletion to program repair, and developed a framework for improving understanding of autocompletion tools to help researchers' understanding and developers' trust.
\end{flushleft}

% \begin{flushleft}
% Through numerous empirical evaluations, of which included user studies and specially designed benchmarks, we show the usefulness, practicality, and performance of these works.
% \end{flushleft}
\end{large}

==> acknowledge.tex <==
\begin{large}
\begin{flushleft}
\noindent This dissertation was not performed in a bubble. It was the culmination of constant learning from and support by friends, family, and coworkers. First I would like to generously thank my Ph.D. advisor Denys Poshyvanyk for his guidance and support. He was especially supportive during personal strife and challenges during my Ph.D. Additionally, Denys consistently pushed me to do my best research and offered advise and guidance when needed. This dissertation would not be possible without his invaluable feedback. Thank you, Denys!
\\
\end{flushleft}

\begin{flushleft}
\noindent Additionally, I would like to thank my lab members, David Nader Palacio, Kevin Moran, Amit Ami, Carlos Bernal-Cardenas, Cody Watson, Michele Tufano, and Yanfu Yan, for their friendship and invaluable knowledge they shared with me. I would also like to thank my Ph.D. committee members, Dr. Oscar Chaparro, Dr. Adwait Nadkarni, Dr. Huajie Shao, and Dr. Robert Lewis for their extremely valuable feedback.
\\
\end{flushleft}

\begin{flushleft}
\noindent I would also like to extend my thanks to my collaborators Antonio Mastropaolo, Rosalia Tufano, Emad Aghajani, Dr. Gabriele Bavota, Dr. Massimiliano Di Penta, Dr. Andrian Marcus, and many others. It is a pleasure to collaborate with each of them and I hope to continue collaboration. \\
\end{flushleft}

\begin{flushleft}
\noindent Lastly, I would like to thank my family and friends for the continued support, especially my mom who always believed in me.\\
\end{flushleft}

\end{large}

==> macro.tex <==
\makeatletter

% Tango
% --------------------------
\newcommand{\tango}{{\textsc{Tango}}\xspace}
\newcommand{\tangos}{{\textsc{Tango}'s}\xspace}
\newcommand{\tangolong}{{\sc de\textbf{T}ecting duplic\textbf{A}te scree\textbf{N} recordin\textbf{G}s of s\textbf{O}ftware bugs}\xspace}
\newcommand{\tangot}{{\sc Tango$_{txt}$}\xspace}
\newcommand{\tangov}{{\sc Tango$_{vis}$}\xspace}
\newcommand{\tangoc}{{\sc Tango$_{comb}$}\xspace}
\newcommand{\bflcs}{B+f-LCS\xspace}
\newcommand{\bwlcs}{B+w-LCS\xspace}
% --------------------------

% Athena
% --------------------------
\newcommand\athena{\textsc{Athena}\xspace}
\newcommand\athenas{\textsc{Athena's}\xspace}
\newcommand{\imrepos}{\textcolor{black}{$25$}\xspace}
\newcommand{\imcommits}{\textcolor{black}{$910$}\xspace}
\newcommand{\imtasks}{\textcolor{red}{$XX$}\xspace}
% --------------------------

% DLSLR
% --------------------------
\newcommand\revision[1]{{\color{black}{#1}}}
\newcommand{\mybox}[4]{
    \begin{figure}[h!]
        \centering
    \begin{tikzpicture}
        \node[anchor=text,text width=\columnwidth-1.2cm, draw, rounded corners, line width=1pt, fill=#3, inner sep=5mm] (big) {\\#4};
        \node[draw, rounded corners, line width=.5pt, fill=#2, anchor=west, xshift=5mm] (small) at (big.north west) {#1};
    \end{tikzpicture}
    \end{figure}
}

\newcommand{\includedpapers}{128}
\newcommand{\includedsetasks}{23}
\newcommand{\add}[1]{{\leavevmode\color{black}{\xspace#1}}}
\definecolor{lightgrey}{HTML}{d3d3d3}
\newtcolorbox{resultbox}{colback=lightgrey, arc=0.5mm, top=2mm, bottom=2mm, left=2mm, right=2mm}


\newcommand{\onehotcount}{$\approx6\%$}
\newcommand{\neuralcount}{$\approx35\%$}
\newcommand{\tokcount}{$\approx51\%$}

\newcommand{\naoverfitcount}{$\approx19\%$}
\newcommand{\dropoutcount}{$\approx32\%$}
\newcommand{\earlycount}{$\approx13\%$}
\newcommand{\cleancount}{$\approx14\%$}
\newcommand{\regcount}{$\approx15\%$}

\newcommand{\rnncount}{$\approx45\%$}
\newcommand{\cnncount}{$\approx21\%$}
\newcommand{\encdeccount}{$\approx22\%$}
\newcommand{\autocount}{$\approx8\%$}
\newcommand{\siamcount}{$\approx5\%$}
\newcommand{\fnncount}{$\approx13\%$}

\newcommand{\entropycount}{$\approx20\%$}
\newcommand{\binentropycount}{$\approx5\%$}
\newcommand{\neglogcount}{$\approx9\%$}
\newcommand{\maxlogcount}{$\approx9\%$}
\newcommand{\cosinelog}{$\approx2\%$}

\newcommand{\adadeltacount}{3}
\newcommand{\adamcount}{30}
\newcommand{\rmspropcount}{11}
\newcommand{\adagradcount}{3}

\newcommand{\accpercent}{$\approx46\%$}
\newcommand{\precpercent}{$\approx35\%$}
\newcommand{\recallpercent}{$\approx33\%$}
\newcommand{\fpercent}{$\approx26\%$}

\newcommand{\replipercent}{$\approx14\%$}
\newcommand{\replicount}{$19$}
\newcommand{\reprodpercent}{$\approx49\%$}
\newcommand{\reprodcount}{$63$}

\newcommand{\learnalgocount}{$37$}
\newcommand{\hypercount}{\textbf{$45$}}

%%%% Sampling Macros
\newcommand{\diffpopulation}{0.02 }
\newcommand{\diffstratified}{0.48 $\pm$ 0.32 }
\newcommand{\diffmedian}{0.13 }

\newcommand{\stringtotal}{1,771 }
\newcommand{\inclusiontotal}{1,217 }
\newcommand{\samplingtotal}{125 }
\newcommand{\nonsamplingtotal}{128 }
% --------------------------


% this  is a easy way to add and highlight new text  ...
% just comment in/out the \tnew macro ..

\def\signed#1{{\unskip\nobreak\hfil\penalty50
    \hskip2em\hbox{}\nobreak\hfil\sl#1
    \parfillskip=0pt \finalhyphendemerits=0 \par}}

\newcommand{\tnew}[1]{{\bf { #1 }} }
%\newcommand{\tnew}[1]{{ { #1 }} }

% math and theorem definition

\newcommand{\ndef}{\stackrel{\rm def}{=}}
\newcommand\REF{{\color{red} \textbf{[REFS]}}\xspace}
\newcommand{\figref}[1]{Figure~\ref{#1}\xspace}
\newcommand{\tabref}[1]{Table~\ref{#1}\xspace}

% this is used for draft only

%\renewcommand{\baselinestretch}{2}

% just to number pages in the draft

\useunder{\uline}{\ul}{}

% nothing i.e., no-numbering final and camera ready

%\pagestyle{empty}


\newsavebox\CBox
\newlength\CLength
\def\circled#1{\sbox\CBox{#1}%
  \ifdim\wd\CBox>\ht\CBox \CLength=\wd\CBox\else\CLength=\ht\CBox\fi
    \makebox[1.2\CLength]{\makebox(0,0.9\CLength){\put(0,0){\circle{1.3\CLength}}}%
    \makebox(0,1.0\CLength){\put(-.5\wd\CBox,0){#1}}}}

\def\circledlong#1{\sbox\CBox{#1}%
  \ifdim\wd\CBox>\ht\CBox \CLength=\wd\CBox\else\CLength=\ht\CBox\fi
    \makebox[1.2\CLength]{\makebox(0,0.6\CLength){\put(0,0){\circle{1.3\CLength}}}%
    \makebox(0,0.6\CLength){\put(-.5\wd\CBox,0){#1}}}}

\lstset{
	basicstyle=\footnotesize\ttfamily,
	breaklines=true,
    frame=tb, % draw a frame at the top and bottom of the code block
    tabsize=4, % tab space width
    showstringspaces=false, % don't mark spaces in strings
    numbers=left, % display line numbers on the left
    commentstyle=\color{Red}, % comment color
    keywordstyle=\color{blue}, % keyword color
    stringstyle=\color{OliveGreen}, % string color
	xleftmargin=.25in %align numbers to left side
}

\newboolean{showcomments}


\setboolean{showcomments}{true}

\ifthenelse{\boolean{showcomments}}
  {\newcommand{\nb}[2]{
    \fbox{\bfseries\sffamily\scriptsize#1}
    {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
   }
   \newcommand{\cvsversion}{\emph{\scriptsize$-$Id: macro.tex,v 1.9 2005/12/09 22:38:33 giulio Exp $}}
  }
  {\newcommand{\nb}[2]{}
   \newcommand{\cvsversion}{}
  }

\newcommand\nathan[1]{{\color{purple} \nb{NATHAN}{#1}}}
\newcommand\denys[1]{{\color{blue} \nb{DENYS}{#1}}}

\newcommand\new[1]{{\textcolor{black}{#1}}}

\newcommand{\ie}{\textit{i.e.},\xspace}
\newcommand{\eg}{\textit{e.g.},\xspace}
\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\aka}{\textit{a.k.a.}\xspace}

\newcommand\NEW[1]{\nb{NEW}{#1}}






==> tabs/tango/all_apps_best.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{|l|c|c|c|c||c|c|c|c|c|c|c|}
    \hline
    \multicolumn{5}{|l||}{Configurations}                                 & \multicolumn{7}{c|}{Metrics}  \\
    \hline
    App & Model  & Approach  & FTK & VWs & mRR  & mAP & $\mu$ Rank & Rank $\sigma$ & HIT@1 & HIT@3  & HIT@5  \\
    \hline
    APOD & SIFT & w-lcs & 1 & 10k & 64.6\% & 51.1\% & 3.0 & 3.2 & 47.7\% & 78.5\% & 80.0\% \\
    APOD & SimCLR & bovw & 5 & 1k & 80.0\% & 66.8\% & 1.7 & 1.3 & 68.1\% & 91.5\% & 97.8\% \\
    APOD & OCR\&IR & all-text & 1 & N/A & 81.8\% & 74.2\% & 1.4 & 0.7 & 67.2\% & 98.0\% & 99.9\% \\
    \hline
    DROID & SIFT & w-lcs & 1 & 10k & 66.3\% & 55.0\% & 2.5 & 2.3 & 49.1\% & 80.1\% & 88.4\% \\
    DROID & SimCLR & bovw & 5 & 10k & 72.3\% & 61.4\% & 2.3 & 2.0 & 59.3\% & 78.1\% & 89.4\% \\
    DROID & OCR\&IR & uni-f & 5 & N/A & 72.4\% & 66.0\% & 2.0 & 1.5 & 55.9\% & 85.2\% & 95.1\% \\
    \hline
    GNU & SIFT & w-lcs & 1 & 10k & 66.1\% & 57.2\% & 2.2 & 1.6 & 47.4\% & 81.2\% & 94.2\% \\
    GNU & SimCLR & bovw & 5 & 5k & 82.9\% & 72.5\% & 1.5 & 1.0 & 71.5\% & 94.4\% & 99.9\% \\
    GNU & OCR\&IR & uni-w & 5 & N/A & 85.2\% & 78.8\% & 1.3 & 0.5 & 71.6\% & 99.8\% & 100.0\% \\
    \hline
    GROW & SIFT & bovw & 5 & 1k & 74.5\% & 67.3\% & 2.3 & 2.2 & 64.0\% & 81.1\% & 88.3\% \\
    GROW & SimCLR & bovw & 5 & 5k & 77.4\% & 75.1\% & 1.9 & 1.7 & 65.1\% & 87.9\% & 95.7\% \\
    GROW & OCR\&IR & all-text & 1 & N/A & 77.4\% & 70.8\% & 1.9 & 1.7 & 64.1\% & 90.7\% & 94.6\% \\
    \hline
    TIME & SIFT & w-lcs & 1 & 5k & 49.9\% & 40.9\% & 3.2 & 2.4 & 26.4\% & 68.3\% & 86.7\% \\
    TIME & SimCLR & bovw & 5 & 1k & 74.8\% & 67.6\% & 2.3 & 2.4 & 63.7\% & 80.9\% & 90.1\% \\
    TIME & OCR\&IR & all-text & 5 & N/A & 47.4\% & 37.7\% & 4.0 & 3.1 & 28.3\% & 57.0\% & 70.6\% \\
    \hline
    TOK & SIFT & w-lcs & 5 & 5k & 44.3\% & 35.9\% & 4.2 & 3.2 & 24.4\% & 52.0\% & 73.0\% \\
    TOK & SimCLR & bovw & 5 & 1k & 77.7\% & 69.3\% & 1.6 & 0.9 & 60.6\% & 96.4\% & 99.8\% \\
    TOK & OCR\&IR & all-text & 5 & N/A & 61.3\% & 53.3\% & 2.6 & 2.1 & 42.6\% & 77.0\% & 88.4\% \\
    \hline
    \hline
    ALL & SIFT & w-lcs & 1 & 10k & 56.9\% & 47.7\% & 3.1 & 2.6 & 37.4\% & 57.3\% & 70.7\% & 78.3\% & 83.0\% \\
    ALL & SimCLR & bovw & 5 & 1k & 75.3\% & 67.8\% & 1.9 & 1.7 & 61.6\% & 78.0\% & 86.7\% & 91.3\% & 95.0\% \\
    ALL & OCR\&IR & all-text & 5 & N/A & 69.8\% & 63.7\% & 2.3 & 2.1 & 54.1\% & 72.6\% & 82.6\% & 87.6% & 90.8\% \\
    \hline
    \end{tabular}
    \newline
    \caption{Top Configurations per model per app \NATHAN{TODO: Remove standard deviation, fix }}
    \label{tab:all_best}
\end{table*}

==> tabs/tango/all_apps_best_combined.tex <==
% \begin{table*}[]
% \centering
% \caption{Top Configuration per combined model per app}
% \label{tab:all_best_combined_ocr}
% \begin{tabular}{c|c|ccc|ccccc}
% \hline
% \textbf{App}             & \textbf{W}                     & \textbf{mRR} & \textbf{mAP} & \textbf{μ Rank} & \textbf{H@1} & \textbf{H@2} & \textbf{H@3} & \textbf{H@4} & \textbf{H@5} \\ \hline
% APOD                     & 0.8 / 0.2                      & 84.4\%       & 75.8\%       & 1.4             & 73.1\%       & 87.9\%       & 98.5\%       & 99.9\%       & 100.0\%      \\ %\hline
% APOD                     & 1.0 / 0.0                      & 80.0\%       & 66.8\%       & 1.7             & 68.1\%       & 82.6\%       & 91.5\%       & 93.3\%       & 97.8\%       \\ %\hline
% APOD                     & 0.0 / 1.0                      & 80.8\%       & 75.3\%       & 1.5             & 65.7\%       & 88.6\%       & 98.3\%       & 99.1\%       & 100.0\%      \\ \hline
% DROID                    & 0.8 / 0.2                      & 70.6\%       & 66.7\%       & 2.2             & 55.9\%       & 71.0\%       & 80.7\%       & 89.3\%       & 93.6\%       \\ %\hline
% DROID                    & 1.0 / 0.0                      & 64.6\%       & 59.2\%       & 2.6             & 49.5\%       & 61.7\%       & 72.3\%       & 82.2\%       & 89.0\%       \\ %\hline
% DROID                    & 0.0 / 1.0                      & 67.9\%       & 64.7\%       & 2.3             & 52.0\%       & 69.8\%       & 78.4\%       & 86.9\%       & 91.6\%       \\ \hline
% GNU                      & 0.8 / 0.2                      & 89.5\%       & 84.7\%       & 1.3             & 81.6\%       & 94.2\%       & 96.8\%       & 99.0\%       & 99.6\%       \\ %\hline
% GNU                      & 1.0 / 0.0                      & 81.8\%       & 75.1\%       & 1.6             & 70.1\%       & 85.3\%       & 93.3\%       & 97.0\%       & 98.4\%       \\ %\hline
% GNU                      & 0.0 / 1.0                      & 84.5\%       & 82.3\%       & 1.4             & 72.2\%       & 92.0\%       & 96.9\%       & 99.1\%       & 99.9\%       \\ \hline
% GROW                     & 0.8 / 0.2                      & 81.7\%       & 75.4\%       & 1.7             & 71.4\%       & 82.5\%       & 92.8\%       & 95.6\%       & 96.4\%       \\ %\hline
% GROW                     & 1.0 / 0.0                      & 72.7\%       & 68.8\%       & 2.0             & 57.4\%       & 75.6\%       & 86.0\%       & 90.6\%       & 95.2\%       \\ %\hline
% GROW                     & 0.0 / 1.0                      & 76.8\%       & 69.0\%       & 1.9             & 63.6\%       & 80.1\%       & 87.7\%       & 92.6\%       & 94.4\%       \\ \hline
% TIME                     & 0.8 / 0.2                      & 59.6\%       & 51.7\%       & 2.8             & 40.2\%       & 58.8\%       & 74.7\%       & 84.6\%       & 89.9\%       \\ %\hline
% TIME                     & 1.0 / 0.0                      & 74.8\%       & 67.6\%       & 2.3             & 63.7\%       & 75.9\%       & 80.9\%       & 86.4\%       & 90.1\%       \\ %\hline
% TIME                     & 0.0 / 1.0                      & 47.4\%       & 37.7\%       & 4.0             & 28.3\%       & 44.4\%       & 57.0\%       & 64.0\%       & 70.6\%       \\ \hline
% TOK                      & 0.8 / 0.2                      & 69.8\%       & 60.8\%       & 2.0             & 50.9\%       & 76.9\%       & 85.3\%       & 92.1\%       & 96.0\%       \\ %\hline
% TOK                      & 1.0 / 0.0                      & 77.7\%       & 69.3\%       & 1.6             & 60.6\%       & 86.7\%       & 96.4\%       & 98.1\%       & 99.8\%       \\ %\hline
% TOK                      & 0.0 / 1.0                      & 61.3\%       & 53.3\%       & 2.6             & 42.6\%       & 60.7\%       & 77.0\%       & 84.1\%       & 88.4\%       \\ \hline \hline
% ALL & 0.8 / 0.2 & 75.9\%       & 69.2\%       & 1.9             & 62.2\%       & 78.5\%       & 88.1\%       & 93.4\%       & 95.9\%       \\ %\hline
% ALL & 1.0 / 0.0                      & 75.3\%       & 67.8\%       & 1.9             & 61.6\%       & 78.0\%       & 86.7\%       & 91.3\%       & 95.0\%       \\ %\hline
% ALL & 0.0 / 1.0                      & 69.8\%       & 63.7\%       & 2.3             & 54.1\%       & 72.6\%       & 82.6\%       & 87.6\%       & 90.8\%       \\ \hline
% \end{tabular}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{Top combined configuration, weight 0.8 on visual information and 0.2 on textual information, per app and overall.}
\label{tab:all_best_combined_ocr}
\begin{tabular}{c|l|ccc|ccccc}
\textbf{App}           & \textbf{Info Type}                   & \textbf{mRR} & \textbf{mAP} & \textbf{μ Rank} & \textbf{H@1} & \textbf{H@2} & \textbf{H@3} & \textbf{H@4} & \textbf{H@5} \\ \hline
\multirow{3}{*}{APOD}  & \tango_{vis + txt} & 84.4\%       & 75.8\%       & 1.4             & 73.1\%       & 87.9\%       & 98.5\%       & 99.9\%       & 100.0\%      \\ \cline{2-10} 
                       & \tango_{vis}       & 80.0\%       & 66.8\%       & 1.7             & 68.1\%       & 82.6\%       & 91.5\%       & 93.3\%       & 97.8\%       \\ \cline{2-10} 
                       & \tango_{txt}       & 80.8\%       & 75.3\%       & 1.5             & 65.7\%       & 88.6\%       & 98.3\%       & 99.1\%       & 100.0\%      \\ \hline
\multirow{3}{*}{DROID} & \tango_{vis + txt} & 70.6\%       & 66.7\%       & 2.2             & 55.9\%       & 71.0\%       & 80.7\%       & 89.3\%       & 93.6\%       \\ \cline{2-10} 
                       & \tango_{vis}       & 64.6\%       & 59.2\%       & 2.6             & 49.5\%       & 61.7\%       & 72.3\%       & 82.2\%       & 89.0\%       \\ \cline{2-10} 
                       & \tango_{txt}       & 67.9\%       & 64.7\%       & 2.3             & 52.0\%       & 69.8\%       & 78.4\%       & 86.9\%       & 91.6\%       \\ \hline
\multirow{3}{*}{GNU}   & \tango_{vis + txt} & 89.5\%       & 84.7\%       & 1.3             & 81.6\%       & 94.2\%       & 96.8\%       & 99.0\%       & 99.6\%       \\ \cline{2-10} 
                       & \tango_{vis}       & 81.8\%       & 75.1\%       & 1.6             & 70.1\%       & 85.3\%       & 93.3\%       & 97.0\%       & 98.4\%       \\ \cline{2-10} 
                       & \tango_{txt}       & 84.5\%       & 82.3\%       & 1.4             & 72.2\%       & 92.0\%       & 96.9\%       & 99.1\%       & 99.9\%       \\ \hline
\multirow{3}{*}{GROW}  & \tango_{vis + txt} & 81.7\%       & 75.4\%       & 1.7             & 71.4\%       & 82.5\%       & 92.8\%       & 95.6\%       & 96.4\%       \\ \cline{2-10} 
                       & \tango_{vis}       & 72.7\%       & 68.8\%       & 2.0             & 57.4\%       & 75.6\%       & 86.0\%       & 90.6\%       & 95.2\%       \\ \cline{2-10} 
                       & \tango_{txt}       & 76.8\%       & 69.0\%       & 1.9             & 63.6\%       & 80.1\%       & 87.7\%       & 92.6\%       & 94.4\%       \\ \hline
\multirow{3}{*}{TIME}  & \tango_{vis + txt} & 59.6\%       & 51.7\%       & 2.8             & 40.2\%       & 58.8\%       & 74.7\%       & 84.6\%       & 89.9\%       \\ \cline{2-10} 
                       & \tango_{vis}       & 74.8\%       & 67.6\%       & 2.3             & 63.7\%       & 75.9\%       & 80.9\%       & 86.4\%       & 90.1\%       \\ \cline{2-10} 
                       & \tango_{txt}       & 47.4\%       & 37.7\%       & 4.0             & 28.3\%       & 44.4\%       & 57.0\%       & 64.0\%       & 70.6\%       \\ \hline
\multirow{3}{*}{TOK}   & \tango_{vis + txt} & 69.8\%       & 60.8\%       & 2.0             & 50.9\%       & 76.9\%       & 85.3\%       & 92.1\%       & 96.0\%       \\ \cline{2-10} 
                       & \tango_{vis}       & 77.7\%       & 69.3\%       & 1.6             & 60.6\%       & 86.7\%       & 96.4\%       & 98.1\%       & 99.8\%       \\ \cline{2-10} 
                       & \tango_{txt}       & 61.3\%       & 53.3\%       & 2.6             & 42.6\%       & 60.7\%       & 77.0\%       & 84.1\%       & 88.4\%       \\ \hline \hline
\multirow{3}{*}{ALL}   & \tango_{vis + txt} & 75.9\%       & 69.2\%       & 1.9             & 62.2\%       & 78.5\%       & 88.1\%       & 93.4\%       & 95.9\%       \\ \cline{2-10} 
                       & \tango_{vis}       & 75.3\%       & 67.8\%       & 1.9             & 61.6\%       & 78.0\%       & 86.7\%       & 91.3\%       & 95.0\%       \\ \cline{2-10} 
                       & \tango_{txt}       & 69.8\%       & 63.7\%       & 2.3             & 54.1\%       & 72.6\%       & 82.6\%       & 87.6\%       & 90.8\%       \\ \hline
\end{tabular}
\end{table*}






% \begin{table*}[]
%     % 
%     % \centering
%     \hspace*{-1.7cm}
%     \centering
%     \begin{tabular}{|l|p{1.6cm}|p{1.2cm}|p{0.7cm}|p{0.8cm}|p{0.7cm}||c|c|c|c|c|c|c|c|c|}
%     %\hline
%     \multicolumn{6}{|l||}{Configurations}                                 & \multicolumn{9}{c|}{Metrics}  \\
%     %\hline
%     App & Model  & Approach  & FTK & VWs & W & mRR  & mAP & $\mu$ Rank & Rank $\sigma$ & H@1 & H@2 & H@3 & H@4 & H@5  \\
%     %\hline
%     % APOD & SIFT / OCR\&IR & w-lcs / all-text & 1 / 5 & 10k / N/A & 0.2 / 0.8 & 81.9\% & 74.5\% & 1.4 & 0.7 & 66.5\% & 92.5\% & 98.8\% & 99.9\% & 100.0\% \\
%     % %\hline
%     % APOD & SIFT / OCR\&IR & w-lcs / all-text & 1 / 5 & 10k / N/A & 1.0 / 0.0 & 67.6\% & 50.4\% & 2.8 & 3.0 & 52.8\% & 70.2\% & 78.3\% & 83.5\% & 86.2\% \\
%     % %\hline
%     APOD & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.8 / 0.2 & 84.4\% & 75.8\% & 1.4 & 0.7 & 73.1\% & 87.9\% & 98.5\% & 99.9\% & 100.0\% \\
%     %\hline
%     APOD & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 1.0 / 0.0 & 80.0\% & 66.8\% & 1.7 & 1.3 & 68.1\% & 82.6\% & 91.5\% & 93.3\% & 97.8\% \\
%     %\hline
%     APOD & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.0 / 1.0 & 80.8\% & 75.3\% & 1.5 & 0.8 & 65.7\% & 88.6\% & 98.3\% & 99.1\% & 100.0\% \\
%     %\hline
%     % DROID & SIFT / OCR\&IR & w-lcs / all-text & 1 / 5 & 10k / N/A & 0.8 / 0.2 & 78.4\% & 66.8\% & 1.8 & 1.6 & 66.9\% & 79.6\% & 87.8\% & 92.1\% & 95.9\% \\
%     % %\hline
%     % DROID & SIFT / OCR\&IR & w-lcs / all-text & 1 / 5 & 10k / N/A & 1.0 / 0.0 & 59.8\% & 53.0\% & 3.0 & 2.6 & 43.3\% & 57.8\% & 68.9\% & 76.2\% & 84.2\% \\
%     % %\hline
%     DROID & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.8 / 0.2 & 70.6\% & 66.7\% & 2.2 & 1.8 & 55.9\% & 71.0\% & 80.7\% & 89.3\% & 93.6\% \\
%     %\hline
%     DROID & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 1.0 / 0.0 & 64.6\% & 59.2\% & 2.6 & 2.1 & 49.5\% & 61.7\% & 72.3\% & 82.2\% & 89.0\% \\
%     %\hline
%     DROID & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.0 / 1.0 & 67.9\% & 64.7\% & 2.3 & 2.0 & 52.0\% & 69.8\% & 78.4\% & 86.9\% & 91.6\% \\
%     %\hline
%     % GNU & SIFT / OCR\&IR & w-lcs / all-text & 1 / 5 & 10k / N/A & 0.8 / 0.2 & 85.0\% & 81.4\% & 1.4 & 0.7 & 73.6\% & 90.5\% & 97.3\% & 99.6\% & 100.0\% \\
%     % %\hline
%     % GNU & SIFT / OCR\&IR & w-lcs / all-text & 1 / 5 & 10k / N/A & 1.0 / 0.0 & 56.5\% & 52.2\% & 2.6 & 1.7 & 33.8\% & 57.2\% & 75.3\% & 84.2\% & 91.4\% \\
%     % %\hline
%     GNU & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.8 / 0.2 & 89.5\% & 84.7\% & 1.3 & 0.7 & 81.6\% & 94.2\% & 96.8\% & 99.0\% & 99.6\% \\
%     %\hline
%     GNU & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 1.0 / 0.0 & 81.8\% & 75.1\% & 1.6 & 1.1 & 70.1\% & 85.3\% & 93.3\% & 97.0\% & 98.4\% \\
%     %\hline
%     GNU & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.0 / 1.0 & 84.5\% & 82.3\% & 1.4 & 0.8 & 72.2\% & 92.0\% & 96.9\% & 99.1\% & 99.9\% \\
%     %\hline
%     % GROW & SIFT / OCR\&IR & w-lcs / all-text & 1 / 5 & 10k / N/A & 0.8 / 0.2 & 82.2\% & 73.5\% & 1.5 & 0.8 & 69.8\% & 85.6\% & 96.9\% & 99.4\% & 99.9\% \\
%     % %\hline
%     % GROW & SIFT / OCR\&IR & w-lcs / all-text & 1 / 5 & 10k / N/A & 1.0 / 0.0 & 64.1\% & 56.1\% & 2.5 & 2.0 & 47.3\% & 63.8\% & 74.9\% & 84.0\% & 88.6\% \\
%     % %\hline
%     GROW & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.7 / 0.3 & 81.9\% & 74.8\% & 1.7 & 1.5 & 72.0\% & 82.6\% & 91.7\% & 95.2\% & 96.5\% \\
%     %\hline
%     GROW & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 1.0 / 0.0 & 72.7\% & 68.8\% & 2.0 & 1.7 & 57.4\% & 75.6\% & 86.0\% & 90.6\% & 95.2\% \\
%     %\hline
%     GROW & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.0 / 1.0 & 76.8\% & 69.0\% & 1.9 & 1.6 & 63.6\% & 80.1\% & 87.7\% & 92.6\% & 94.4\% \\
%     %\hline
%     % TIME & SIFT / OCR\&IR & w-lcs / all-text & 1 / 5 & 10k / N/A & 0.9 / 0.1 & 49.5\% & 39.7\% & 3.2 & 2.3 & 26.0\% & 46.8\% & 67.8\% & 79.0\% & 85.2\% \\
%     % %\hline
%     % TIME & SIFT / OCR\&IR & w-lcs / all-text & 1 / 5 & 10k / N/A & 1.0 / 0.0 & 39.0\% & 33.4\% & 4.0 & 2.6 & 14.1\% & 35.9\% & 52.7\% & 66.0\% & 73.5\% \\
%     % %\hline
%     TIME & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.9 / 0.1 & 63.2\% & 58.1\% & 2.6 & 2.3 & 43.1\% & 66.3\% & 82.1\% & 89.5\% & 92.1\% \\
%     %\hline
%     TIME & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 1.0 / 0.0 & 74.8\% & 67.6\% & 2.3 & 2.4 & 63.7\% & 75.9\% & 80.9\% & 86.4\% & 90.1\% \\
%     %\hline
%     TIME & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.0 / 1.0 & 47.4\% & 37.7\% & 4.0 & 3.1 & 28.3\% & 44.4\% & 57.0\% & 64.0\% & 70.6\% \\
%     %\hline
%     % TOK & SIFT / OCR\&IR & w-lcs / all-text & 1 / 5 & 10k / N/A & 0.1 / 0.9 & 58.4\% & 52.0\% & 2.8 & 2.2 & 38.9\% & 58.6\% & 72.7\% & 79.8\% & 84.9\% \\
%     % %\hline
%     % TOK & SIFT / OCR\&IR & w-lcs / all-text & 1 / 5 & 10k / N/A & 1.0 / 0.0 & 38.0\% & 31.2\% & 4.6 & 3.1 & 17.0\% & 31.1\% & 47.2\% & 59.8\% & 64.9\% \\
%     % %\hline
%     TOK & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.9 / 0.1 & 70.3\% & 63.0\% & 1.9 & 1.3 & 51.4\% & 76.2\% & 88.4\% & 94.3\% & 97.4\% \\
%     %\hline
%     TOK & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 1.0 / 0.0 & 77.7\% & 69.3\% & 1.6 & 0.9 & 60.6\% & 86.7\% & 96.4\% & 98.1\% & 99.8\% \\
%     %\hline
%     TOK & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.0 / 1.0 & 61.3\% & 53.3\% & 2.6 & 2.1 & 42.6\% & 60.7\% & 77.0\% & 84.1\% & 88.4\% \\
%     %\hline
%     %\hline
%     ALL & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.9 / 0.1 & 76.0\% & 70.0\% & 1.9 & 1.6 & 62.6\% & 78.6\% & 87.3\% & 92.6\% & 95.1\% \\
%     %\hline
%     ALL & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 1.0 / 0.0 & 75.3\% & 67.8\% & 1.9 & 1.7 & 61.6\% & 78.0\% & 86.7\% & 91.3\% & 95.0\% \\
%     %\hline
%     ALL & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.0 / 1.0 & 69.8\% & 63.7\% & 2.3 & 2.1 & 54.1\% & 72.6\% & 82.6\% & 87.6\% & 90.8\% \\
%     % %\hline
%     % SPLIT & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & (0.8 / 0.2) / (1.0 / 0.0) & 79.8\% & 73.2\% & 1.7 & 1.5 & 67.7\% & 83.0\% & 91.0\% & 94.7\% & 96.6\% \\
%     %\hline
%     \end{tabular}
%     \newline
%     \caption{Top Configurations per combined model per app \NATHAN{Not sure if having this table be so close to the edges violates any format rules. May need to drop some of the Hits} \NATHAN{TODO: Remove standard deviation}}
%     \label{tab:all_best_combined_ocr}
% \end{table*}

==> tabs/tango/apod.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{4}{|c|}{Configurations}                           & \multicolumn{7}{c|}{Metrics}                                                                \\
    \hline
    Model  & Approach  & FTK & VWs & mRR  & mAP & $\mu$ Rank & Rank \sigma  & HIT@1  & HIT@3  & HIT@5  \\
    \hline
     SIFT & w-lcs & 1 & 10,000      & 64.62\% & 51.14\% & 3.02 & 3.15  & 47.7\% & 78.5\% & 80.0\%   \\
     SIFT & bovw & 5 &  5,000              & 64.05\% & 53.42\% & 2.75 & 2.60  & 47.3\% & 75.9\% & 85.7\%   \\
     SIFT & bovw & 5 &  10,000             & 63.09\% & 52.88\% & 2.62 & 2.27  & 45.3\% & 76.7\% & 89.6\%   \\
     SIFT & w-lcs & 5 & 1,000       & 62.81\% & 52.09\% & 2.52 & 2.18  & 42.2\% & 79.6\% & 91.0\%   \\
     SIFT & w-lcs & 1 & 1,000       & 62.31\% & 47.51\% & 2.28 & 1.53  & 40.1\% & 83.2\% & 95.8\%   \\
     SIFT & w-lcs & 5 & 10,000      & 62.05\% & 52.99\% & 2.71 & 2.23  & 44.4\% & 73.5\% & 85.6\%   \\
     \hline
    SimCLR  & bovw  & 5  & 1,000               & 80.03\% & 66.77\% & 1.68 & 1.27  & 68.1\% & 91.5\% & 97.8\%    \\
    SimCLR  & bovw  & 5  & 5,000               & 76.27\% & 68.31\% & 2.14 & 2.27  & 64.9\% & 83.2\% & 91.2\%    \\
    SimCLR  & bovw  & 5  & 10,000              & 75.10\% & 69.22\% & 1.94 & 1.65  & 61.1\% & 88.5\% & 94.9\%    \\
    SimCLR  & bovw  & 1  & 5,000               & 68.68\% & 62.28\% & 2.59 & 2.64  & 54.2\% & 78.3\% & 87.8\%    \\
    SimCLR  & bovw  & 1  & 1,000               & 67.23\% & 58.64\% & 2.25 & 1.88  & 49.1\% & 83.3\% & 94.4\%    \\
    SimCLR  & bovw  & 1  & 10,000              & 66.75\% & 58.12\% & 2.26 & 1.90  & 47.0\% & 84.4\% & 92.6\%    \\
    \hline
    OCR\&IR & all-text & 1 & N/A              & 81.79\% & 74.18\% & 1.45 & 0.74  & 67.2\% & 98.0\% & 99.9\%    \\
    OCR\&IR & all-text & 5 & N/A              & 80.76\% & 75.32\% & 1.48 & 0.77  & 65.7\% & 98.3\% & 100.0\%   \\
    OCR\&IR & uni-f & 5 & N/A         & 76.52\% & 69.00\% & 1.67 & 0.99  & 60.5\% & 93.2\% & 99.6\%    \\
    OCR\&IR & uni-f & 1 & N/A         & 74.36\% & 67.73\% & 1.68 & 0.90  & 55.3\% & 95.1\% & 100.0\%   \\
    OCR\&IR & uni-w & 5 & N/A          & 73.21\% & 65.10\% & 1.80 & 1.13  & 55.4\% & 91.2\% & 99.0\%    \\
    OCR\&IR & uni-w & 1 & N/A          & 71.07\% & 64.25\% & 1.89 & 1.18  & 52.8\% & 90.2\% & 98.8\%    \\
    \hline
    \end{tabular}
    \newline
    \caption{APOD-SIFT: Keeping only top 6 results due to space contraints}
    \label{tab:apod_top}
\end{table*}

==> tabs/tango/apod_m00.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{4}{|c|}{Configurations}                           & \multicolumn{8}{c|}{Metrics}                                                                \\
    \hline
    Model  & Approach  & FTK & \# of VWs & $\mu$ Rank & Median Rank & Rank \sigma & mRR  & mAP  & HIT@1  & HIT@3  & HIT@5  \\
    \hline
     SIFT & weighted lcs & 1 & 10,000      & 64.62\% & 51.14\% & 3.02 & 3.15 & 2.00 & 47.7\% & 78.5\% & 80.0\%   \\
     SIFT & bovw & 5 &  5,000              & 64.05\% & 53.42\% & 2.75 & 2.60 & 2.00 & 47.3\% & 75.9\% & 85.7\%   \\
     SIFT & bovw & 5 &  10,000             & 63.09\% & 52.88\% & 2.62 & 2.27 & 2.00 & 45.3\% & 76.7\% & 89.6\%   \\
     SIFT & weighted lcs & 5 & 1,000       & 62.81\% & 52.09\% & 2.52 & 2.18 & 2.00 & 42.2\% & 79.6\% & 91.0\%   \\
     SIFT & weighted lcs & 1 & 1,000       & 62.31\% & 47.51\% & 2.28 & 1.53 & 2.00 & 40.1\% & 83.2\% & 95.8\%   \\
     SIFT & weighted lcs & 5 & 10,000      & 62.05\% & 52.99\% & 2.71 & 2.23 & 2.00 & 44.4\% & 73.5\% & 85.6\%   \\
    \hline
    %  SIFT & 1000 & 5 & lcs                & 61.70\% & 54.33\% & 2.87 & 2.56 & 2.00 & 45.3\% & 69.1\% & 87.2\%   \\
    %  SIFT & 5000 & 1 & weighted lcs       & 61.55\% & 47.70\% & 2.96 & 2.80 & 2.00 & 43.5\% & 75.3\% & 83.5\%   \\
    %  SIFT & 5000 & 1 & bovw               & 61.31\% & 45.93\% & 3.09 & 2.97 & 2.00 & 45.3\% & 70.5\% & 84.2\%   \\
    %  SIFT & 5000 & 5 & weighted lcs       & 61.13\% & 53.65\% & 2.82 & 2.46 & 2.00 & 42.2\% & 74.2\% & 84.6\%   \\
    %  SIFT & 1000 & 5 & bovw               & 58.54\% & 51.57\% & 3.06 & 2.53 & 2.00 & 42.0\% & 64.6\% & 83.1\%   \\
    %  SIFT & 10000 & 1 & bovw              & 55.97\% & 43.02\% & 3.23 & 2.96 & 2.00 & 35.3\% & 69.6\% & 84.6\%   \\
    %  SIFT & 1000 & 1 & lcs                & 53.94\% & 41.73\% & 3.25 & 2.87 & 2.00 & 32.3\% & 69.0\% & 85.7\%   \\
    %  SIFT & 1000 & 1 & bovw               & 53.14\% & 42.79\% & 3.46 & 2.89 & 2.00 & 33.5\% & 64.7\% & 79.1\%   \\
    %  SIFT & 10000 & 5 & lcs               & 52.02\% & 45.94\% & 3.19 & 2.29 & 2.00 & 30.5\% & 60.4\% & 83.7\%   \\
    %  SIFT & 5000 & 5 & lcs                & 51.69\% & 46.16\% & 3.58 & 2.93 & 2.00 & 31.7\% & 61.9\% & 75.9\%   \\
    %  SIFT & 10000 & 1 & lcs               & 49.90\% & 40.59\% & 3.57 & 2.99 & 2.00 & 27.8\% & 63.2\% & 83.0\%   \\
    %  SIFT & 5000 & 1 & lcs                & 49.58\% & 40.43\% & 3.70 & 3.10 & 3.00 & 28.5\% & 64.7\% & 78.4\%   \\
    \end{tabular}
    \caption{APOD-SIFT: Keeping only top 6 results due to space contraints}
    \label{tab:apod m00}
\end{table*}

% \begin{table*}[]
%     \centering
%     \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
%     \hline
%     \multicolumn{4}{|c|}{Configurations}                           & \multicolumn{8}{c|}{Metrics}                                                                \\
%     \hline
%     Model  & Approach  & FTK & \# of VWs & $\mu$ Rank & Median Rank & Rank \sigma & mRR  & mAP  & HIT@1  & HIT@3  & HIT@5  \\
    % \hline
%     \hline
%     \end{tabular}
%     \caption{Keeping only top 6 results due to space contraints}
%     \label{tab:apod m00}
% \end{table*}

==> tabs/tango/apod_m01.tex <==
% \begin{tabular}{l|c|c|c|c|c|c|c|c}
% SimCLR  & 1000  & 5  & bovw               & 80.03\% & 66.77\% & 1.68 & 1.27 & 1.00 & 68.1\% & 91.5\% & 97.8\%    \\
% SimCLR  & 5000  & 5  & bovw               & 76.27\% & 68.31\% & 2.14 & 2.27 & 1.00 & 64.9\% & 83.2\% & 91.2\%    \\
% SimCLR  & 10000  & 5  & bovw              & 75.10\% & 69.22\% & 1.94 & 1.65 & 1.00 & 61.1\% & 88.5\% & 94.9\%    \\
% SimCLR  & 5000  & 1  & bovw               & 68.68\% & 62.28\% & 2.59 & 2.64 & 1.00 & 54.2\% & 78.3\% & 87.8\%    \\
% SimCLR  & 1000  & 1  & bovw               & 67.23\% & 58.64\% & 2.25 & 1.88 & 2.00 & 49.1\% & 83.3\% & 94.4\%    \\
% SimCLR  & 10000  & 1  & bovw              & 66.75\% & 58.12\% & 2.26 & 1.90 & 2.00 & 47.0\% & 84.4\% & 92.6\%    \\
% SimCLR  & 10000  & 5  & lcs               & 60.65\% & 55.08\% & 2.67 & 2.28 & 2.00 & 40.5\% & 79.3\% & 89.4\%    \\
% SimCLR  & 1000  & 5  & lcs                & 60.65\% & 55.08\% & 2.67 & 2.28 & 2.00 & 40.5\% & 79.3\% & 89.4\%    \\
% SimCLR  & 5000  & 5  & lcs                & 60.65\% & 55.08\% & 2.67 & 2.28 & 2.00 & 40.5\% & 79.3\% & 89.4\%    \\
% SimCLR  & 10000  & 1  & weighted_lcs      & 59.07\% & 46.59\% & 3.13 & 3.03 & 2.00 & 38.8\% & 77.7\% & 82.2\%    \\
% SimCLR  & 1000  & 1  & weighted_lcs       & 59.07\% & 46.59\% & 3.13 & 3.03 & 2.00 & 38.8\% & 77.7\% & 82.2\%    \\
% SimCLR  & 5000  & 1  & weighted_lcs       & 59.07\% & 46.59\% & 3.13 & 3.03 & 2.00 & 38.8\% & 77.7\% & 82.2\%    \\
% SimCLR  & 10000  & 5  & weighted_lcs      & 55.01\% & 44.85\% & 3.27 & 2.72 & 2.00 & 35.7\% & 65.2\% & 83.7\%    \\
% SimCLR  & 1000  & 5  & weighted_lcs       & 55.01\% & 44.85\% & 3.27 & 2.72 & 2.00 & 35.7\% & 65.2\% & 83.7\%    \\
% SimCLR  & 5000  & 5  & weighted_lcs       & 55.01\% & 44.85\% & 3.27 & 2.72 & 2.00 & 35.7\% & 65.2\% & 83.7\%    \\
% SimCLR  & 10000  & 1  & lcs               & 52.85\% & 44.69\% & 3.19 & 2.41 & 2.00 & 32.1\% & 64.8\% & 84.2\%    \\
% SimCLR  & 1000  & 1  & lcs                & 52.85\% & 44.69\% & 3.19 & 2.41 & 2.00 & 32.1\% & 64.8\% & 84.2\%    \\
% SimCLR  & 5000  & 1  & lcs                & 52.85\% & 44.69\% & 3.19 & 2.41 & 2.00 & 32.1\% & 64.8\% & 84.2\%    \\
% \end{tabular}

\begin{table*}[]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{4}{|c|}{Configurations}                           & \multicolumn{8}{c|}{Metrics}                                                                \\
    \hline
    Model  & Approach  & FTK & \# of VWs & $\mu$ Rank & Median Rank & Rank \sigma & mRR  & mAP  & HIT@1  & HIT@3  & HIT@5  \\
    \hline
    SimCLR  & bovw  & 5  & 1,000               & 80.03\% & 66.77\% & 1.68 & 1.27 & 1.00 & 68.1\% & 91.5\% & 97.8\%    \\
    SimCLR  & bovw  & 5  & 5,000               & 76.27\% & 68.31\% & 2.14 & 2.27 & 1.00 & 64.9\% & 83.2\% & 91.2\%    \\
    SimCLR  & bovw  & 5  & 10,000              & 75.10\% & 69.22\% & 1.94 & 1.65 & 1.00 & 61.1\% & 88.5\% & 94.9\%    \\
    SimCLR  & bovw  & 1  & 5,000               & 68.68\% & 62.28\% & 2.59 & 2.64 & 1.00 & 54.2\% & 78.3\% & 87.8\%    \\
    SimCLR  & bovw  & 1  & 1,000               & 67.23\% & 58.64\% & 2.25 & 1.88 & 2.00 & 49.1\% & 83.3\% & 94.4\%    \\
    SimCLR  & bovw  & 1  & 10,000              & 66.75\% & 58.12\% & 2.26 & 1.90 & 2.00 & 47.0\% & 84.4\% & 92.6\%    \\
    % SimCLR  & 10000  & 5  & lcs               & 60.65\% & 55.08\% & 2.67 & 2.28 & 2.00 & 40.5\% & 79.3\% & 89.4\%    \\
    % SimCLR  & 1000  & 5  & lcs                & 60.65\% & 55.08\% & 2.67 & 2.28 & 2.00 & 40.5\% & 79.3\% & 89.4\%    \\
    % SimCLR  & 5000  & 5  & lcs                & 60.65\% & 55.08\% & 2.67 & 2.28 & 2.00 & 40.5\% & 79.3\% & 89.4\%    \\
    % SimCLR  & 10000  & 1  & weighted_lcs      & 59.07\% & 46.59\% & 3.13 & 3.03 & 2.00 & 38.8\% & 77.7\% & 82.2\%    \\
    % SimCLR  & 1000  & 1  & weighted_lcs       & 59.07\% & 46.59\% & 3.13 & 3.03 & 2.00 & 38.8\% & 77.7\% & 82.2\%    \\
    % SimCLR  & 5000  & 1  & weighted_lcs       & 59.07\% & 46.59\% & 3.13 & 3.03 & 2.00 & 38.8\% & 77.7\% & 82.2\%    \\
    % SimCLR  & 10000  & 5  & weighted_lcs      & 55.01\% & 44.85\% & 3.27 & 2.72 & 2.00 & 35.7\% & 65.2\% & 83.7\%    \\
    % SimCLR  & 1000  & 5  & weighted_lcs       & 55.01\% & 44.85\% & 3.27 & 2.72 & 2.00 & 35.7\% & 65.2\% & 83.7\%    \\
    % SimCLR  & 5000  & 5  & weighted_lcs       & 55.01\% & 44.85\% & 3.27 & 2.72 & 2.00 & 35.7\% & 65.2\% & 83.7\%    \\
    % SimCLR  & 10000  & 1  & lcs               & 52.85\% & 44.69\% & 3.19 & 2.41 & 2.00 & 32.1\% & 64.8\% & 84.2\%    \\
    % SimCLR  & 1000  & 1  & lcs                & 52.85\% & 44.69\% & 3.19 & 2.41 & 2.00 & 32.1\% & 64.8\% & 84.2\%    \\
    % SimCLR  & 5000  & 1  & lcs                & 52.85\% & 44.69\% & 3.19 & 2.41 & 2.00 & 32.1\% & 64.8\% & 84.2\%    \\
    \hline
    \end{tabular}
    \caption{APOD-SimCLR: Keeping only top 6 results due to space contraints}
    \label{tab:apod_m01}
\end{table*}


==> tabs/tango/apod_ocr_ir.tex <==
% \begin{tabular}{l|c|c|c|c|c|c|c|c}
%  OCR \& IR & 1 & all text              & 81.79\% & 74.18\% & 1.45 & 0.74 & 1.00 & 67.2\% & 98.0\% & 99.9\%    \\
%  OCR \& IR & 5 & all text              & 80.76\% & 75.32\% & 1.48 & 0.77 & 1.00 & 65.7\% & 98.3\% & 100.0\%   \\
%  OCR \& IR & 5 & unique frames         & 76.52\% & 69.00\% & 1.67 & 0.99 & 1.00 & 60.5\% & 93.2\% & 99.6\%    \\
%  OCR \& IR & 1 & unique frames         & 74.36\% & 67.73\% & 1.68 & 0.90 & 1.00 & 55.3\% & 95.1\% & 100.0\%   \\
%  OCR \& IR & 5 & unique words          & 73.21\% & 65.10\% & 1.80 & 1.13 & 1.00 & 55.4\% & 91.2\% & 99.0\%    \\
%  OCR \& IR & 1 & unique words          & 71.07\% & 64.25\% & 1.89 & 1.18 & 1.00 & 52.8\% & 90.2\% & 98.8\%    \\
% \end{tabular}

\begin{table*}[]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{4}{|c|}{Configurations}                           & \multicolumn{8}{c|}{Metrics}                                                                \\
    \hline
    Model  & Approach  & FTK & \# of VWs & $\mu$ Rank & Median Rank & Rank \sigma & mRR  & mAP  & HIT@1  & HIT@3  & HIT@5  \\
    \hline
    OCR \& IR & all text & 1 & N/A              & 81.79\% & 74.18\% & 1.45 & 0.74 & 1.00 & 67.2\% & 98.0\% & 99.9\%    \\
    OCR \& IR & all text & 5 & N/A              & 80.76\% & 75.32\% & 1.48 & 0.77 & 1.00 & 65.7\% & 98.3\% & 100.0\%   \\
    OCR \& IR & unique frames & 5 & N/A         & 76.52\% & 69.00\% & 1.67 & 0.99 & 1.00 & 60.5\% & 93.2\% & 99.6\%    \\
    OCR \& IR & unique frames & 1 & N/A         & 74.36\% & 67.73\% & 1.68 & 0.90 & 1.00 & 55.3\% & 95.1\% & 100.0\%   \\
    OCR \& IR & unique words & 5 & N/A          & 73.21\% & 65.10\% & 1.80 & 1.13 & 1.00 & 55.4\% & 91.2\% & 99.0\%    \\
    OCR \& IR & unique words & 1 & N/A          & 71.07\% & 64.25\% & 1.89 & 1.18 & 1.00 & 52.8\% & 90.2\% & 98.8\%    \\
    \hline
    \end{tabular}
    \caption{APOD OCR & IR: Keeping only top 6 results due to space contraints}
    \label{tab:apod_ocr_ir}
\end{table*}

==> tabs/tango/overall_best.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{4}{|l|}{Configurations}                                 & \multicolumn{9}{c|}{Metrics}  \\
    \hline
    Model  & Approach  & FTK & VWs & mRR  & mAP & $\mu$ Rank & Rank $\sigma$ & H@1 & H@2 & H@3 & H@4 & H@5  \\
    \hline
    SIFT & w-lcs & 1 & 10k & 60.7\% & 51.7\% & 2.7 & 2.2 & 41.1\% & 63.1\% & 76.1\% & 81.7\% & 86.5\% \\
    SimCLR & bovw & 5 & 1k & 77.6\% & 70.6\% & 1.8 & 1.4 & 64.3\% & 81.1\% & 89.8\% & 93.7\% & 96.7\% \\
    OCR\&IR & all-text & 1 & N/A & 73.9\% & 68.0\% & 2.0 & 1.8 & 59.3\% & 77.8\% & 85.7\% & 91.3\% & 93.0\% \\
    \hline
    \end{tabular}
    \newline
    \caption{Top Configurations per model across all apps}
    \label{tab:all_best}
\end{table*}

==> tabs/tango/setting2.tex <==
\begin{table}[]
\centering
\small
\caption{Examples of duplicate detection tasks for an app. B$x$-P$y$ represents a bug report from participant $y$ for bug $x$.
% \NATHAN{How does this look for explaining setting 2?}
% \oscar{I like it, but we should simplify it, make it clear, and ideally make it fit in one column.}
} 
\label{tab:setting2}
\setlength\tabcolsep{5pt} 
\begin{tabular}{c|cccccc}

\toprule
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}(Task \#)\\ Query\end{tabular}}} & \multicolumn{6}{c}{\textbf{Corpus}}                                                                                                                                                                                                                                               \\ \cline{2-7} 
                                & \multicolumn{4}{c|}{\textbf{Duplicate Groups}}                                                                                & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Non\\ Duplicates\end{tabular}}}} \\ \cline{2-5}
                                & \multicolumn{2}{c|}{\textbf{Same Bug}} & \multicolumn{2}{c|}{\textbf{Different Bug}} & \multicolumn{2}{c}{}                                                                                   \\ \bottomrule
(1) B1-P1                          & B1-P2                       & \multicolumn{1}{l|}{B1-P3}                      & B2-P1                           & \multicolumn{1}{c|}{...}                           & B3-P1                                               & ...                                              \\
(2) B1-P1                          & B1-P2                       & \multicolumn{1}{l|}{B1-P3}                      & B2-P1                           & \multicolumn{1}{c|}{...}                           & B3-P2                                               & ...                                              \\
(3) B1-P1                          & B1-P2                       & \multicolumn{1}{l|}{B1-P3}                      & B2-P1                           & \multicolumn{1}{c|}{...}                           & B3-P3                                               & ...                                              \\
$\vdots$                             & $\vdots$                             & \multicolumn{1}{c|}{$\vdots$}                            & \vdots                                 & \multicolumn{1}{c|}{$\vdots$}                              & $\vdots$                                                     & $\ddots$                                                 \\ 

%(810) B10-P1                          & B10-P2                       & \multicolumn{1}{l|}{B10-P3}                      & B1-P3                           & \multicolumn{1}{c|}{...}                           & B2-P3                                               & ...                                              \\
\bottomrule
\end{tabular}
\end{table}


% \begin{table*}[]
% \centering
% \caption{Duplication task layout. B\#-P\# represents a bug report of bug \# from participant \#. \NATHAN{How does this look for explaining setting 2?}
% \oscar{I like it, but we should simplify it, make it clear, and ideally make it fit in one column.}
% } 
% \label{tab:setting2}
% \begin{tabular}{c|ccccccccc}
% \toprule
% \multirow{3}{*}{\textbf{Query}} & \multicolumn{9}{c}{\textbf{Corpus}}                                                                                                                   \\ \cline{2-10} 
%                                 & \multicolumn{5}{c|}{\textbf{Duplicate Groups}}                                         & \multicolumn{4}{c}{\multirow{2}{*}{\textbf{Non-Duplicates}}} \\ \cline{2-6}
%                                 & \multicolumn{2}{c|}{\textbf{Same Bug}} & \multicolumn{3}{c|}{\textbf{Different Bug}}   & \multicolumn{4}{c}{}                                         \\ \bottomrule
% B1-P1                          & B1-P2  & \multicolumn{1}{c|}{B1-P3}  & B2-P1 & B2-P2 & \multicolumn{1}{c|}{B2-P3} & B3-P1         & B4-P1         & B5-P1        & ...        \\
% B1-P1                          & B1-P2  & \multicolumn{1}{c|}{B1-P3}  & B2-P1 & B2-P2 & \multicolumn{1}{c|}{B2-P3} & B3-P2         & B4-P2         & B5-P2        & ...        \\
% B1-P1                          & B1-P2  & \multicolumn{1}{c|}{B1-P3}  & B2-P1 & B2-P2 & \multicolumn{1}{c|}{B2-P3} & B3-P3         & B4-P3         & B5-P3        & ...        \\
% $\vdots$                             & $\vdots$        & \multicolumn{1}{c|}{$\vdots$}        & $\vdots$       & \vdots       & \multicolumn{1}{c|}{$\vdots$}       & $\vdots$               &  $\vdots$              & $\vdots$              &  $\ddots$          \\ \bottomrule
% \end{tabular}
% \end{table*}

==> tabs/tango/videos_info_1.tex <==
\begin{table}[]
	\footnotesize
	\centering
	\caption{Touch Indicator Detection Accuracy}
	\label{tab:videos_info_1}
	\begin{tabular}{|l|c|c|c|c|}
		\toprule
		\textbf{App}&\textbf{Avg. Length}&\textbf{Avg. S2R}\\
		\midrule
		APOD	&	\approx21	&	\approx5\\
		GROW	&	\approx22	&	\approx7\\
		TIME	&	\approx25	&	\approx10\\
		TOK	&	\approx22	&	\approx7\\
		DROID	&	\approx24	&	\approx6\\
		GNU	&	\approx39	&	\approx13\\
		\bottomrule
	\end{tabular}
	%\vspace{-0.3cm}
\end{table}

